Attention-based Clinical Note Summarization

In recent years, the trend of deploying digital systems in numerous industries has hiked. The health sector has observed an extensive adoption of digital systems and services that generate significant medical records. Electronic health records contain valuable information for prospective and retrospective analysis that is often not entirely exploited because of the complicated dense information storage. The crude purpose of condensing health records is to select the information that holds most characteristics of the original documents based on a reported disease. These summaries may boost diagnosis and save a doctor's time during a saturated workload situation like the COVID-19 pandemic. In this paper, we are applying a multi-head attention-based mechanism to perform extractive summarization of meaningful phrases on clinical notes. Our method finds major sentences for a summary by correlating tokens, segments, and positional embeddings of sentences in a clinical note. The model outputs attention scores that are statistically transformed to extract critical phrases for visualization on the heat-mapping tool and for human use.

==> body_old.tex <==
% \section{Introduction}
% \label{sec:1}
% Natural language processing (NLP) has been valuable to clinicians in saturated work environments. Health information systems and chatbots have reduced the workload of doctors during the COVID-19 pandemic. Various researches have developed machine learning (ML) models to predict mortality and extract named entity concepts from EHR~\cite{estiri2021predicting}~\cite{10.1093/jamia/ocaa189}.  Presenting text in a shorter form has been practiced in human history long before the birth of computers. A summary is defined as a document that conveys valuable information with significantly less text than usual~\cite{10.1162/089120102762671927}. Summarization can be sensitive in the medical domain owing to the nature of medical abbreviations and technicalities. \par
% The task of summarization can be categorized into two categories from a linguistic perspective. \textit{Extractive} summarization is an indicative approach where phrases are scored based on similarity weights and chosen to produce verbatim. Contrarily,  \textit{abstractive} summarization is an informative approach that requires understanding a topic and generating a new text using fusion and compression. It relies on novel phrases, lexicon, and parsing for language generation~\cite{article}. 

% The notion of presenting a condensed version of a document using computers and algorithms became part of significant research in the late 1950s. Among the first ideas of machine summarization, researchers~\cite{5392672} presented a method for the creation of literature abstracts in exploratory research of IBM Journal. This statistical approach is based on finding word frequency and scoring them based on higher significance. Baxendale et al.~\cite{5392648} came up with the idea based on grammatical position in the text. Other researchers like Lin~\cite{10.3115/990820.990892} and Strzalkowski~\cite{strzalkowski1996natural} proposed query-based summarization that is a direct descendant of information retrieval technique. The method was similar to multi-query vector 
% %is stacked 
% in multi-head attention to performs an effective mapping using a query and a key-value pair to an output.  \par

% Some fundamental questions that arise while summarization are i) which content is essential to select and ii) how to create a shorter version of it ~\cite{inbook}. In this research work, we propose a transformer-based method for selecting meaningful phrases from clinical discharge summaries and extracting them by preserving the sense of clinical notes based on the identified disease. \par

% Transformer~\cite{transformer} is being used as a new tool for text analysis tasks in NLP ~\cite{bahdanau}. 
% % It is a layered neural network-based architecture that exploits attention mechanism for supervised tasks. 
% % Bidirectional Encoder Representation Transformer (BERT) contains 12 transformer layers and several multiple attention heads to form embeddings and attention tensors for a given sentence~\cite{DBLP:journals/corr/abs-1810-04805}. 
% Inspired by~\cite{clinicalbert}, we have further tuned a BERT model utilizing discharge notes classified by diseases of the MIMIC-III dataset, Which captures important syntactic information based on International Classification of Diseases (ICD-9) labels. We extract a discrete attention distribution from the last layer. This probabilistic distribution is later translated using power transforms~\cite{book} to create monotonic data over bell curve~\cite{attentions}. 
% % We choose the value from the first attention head of the last layer to create a series for identifying the importance of every sentence. 
% Finally, the summary is comprised of sentences that have higher attention scores than the mean attention scores.\par

% This paper organizes sections as follows: Section~\ref{sec:2} illustrates various types of extractive summarization approaches and their usescases on medical documents. In Section~\ref{sec:3}, we described the methodology for intended task.
% % we introduce an attention-based method in the medical summarization domain trained on coding clinical notes.
% Section~\ref{sec:4} presents various evaluation methods and states a suitable method for this task. We have displayed results in Section~\ref{sec:5}.
% % with an insight into related work in Section \ref{sec:6}. 
% Finally, we conclude the discussion in Section~\ref{sec:6} with limitations of interpretation in the medical domain in Section~\ref{sec:7}.\par

%%===============
%%===============New Structure of Introduction ==================
%%===============

\section{Introduction}
\label{sec:1}

Presenting text in a shorter form has been practiced in human history long before the birth of computers. A summary is defined as a document that conveys valuable information with significantly less text than usual~\cite{10.1162/089120102762671927}. Summarization can be sensitive in the medical domain owing to the nature of medical abbreviations and technicalities. 
The task of summarization can be categorized into two categories from a linguistic perspective. \textit{Extractive} summarization is an indicative approach where phrases are scored based on similarity weights and chosen to produce verbatim. Contrarily,  \textit{abstractive} summarization is an informative approach that requires understanding a topic and generating a new text using fusion and compression. It relies on novel phrases, lexicon, and parsing for language generation~\cite{article}. 

Natural language processing (NLP) has been valuable to clinicians in saturated work environments. Health information systems and chatbots have reduced the workload of doctors during the COVID-19 pandemic.
% Various researches have developed machine learning (ML) models to predict mortality and extract named entity concepts from EHR~\cite{estiri2021predicting}~\cite{10.1093/jamia/ocaa189}.  
The notion of presenting a condensed version of a document using computers and algorithms became part of significant research in the late 1950s. Among the first ideas of machine summarization, researchers~\cite{5392672} presented a method for the creation of literature abstracts in exploratory research of IBM Journal. This statistical approach is based on finding word frequency and scoring them based on higher significance. Baxendale et al.~\cite{5392648} came up with the idea based on grammatical position in the text. Other researchers like Lin~\cite{10.3115/990820.990892} and Strzalkowski~\cite{strzalkowski1996natural} proposed query-based summarization that is a direct descendant of information retrieval technique. The method was similar to multi-query vector 
%is stacked 
in multi-head attention to performs an effective mapping using a query and a key-value pair to an output.  \par

Some fundamental questions that arise while summarization are i) which content is essential to select and ii) how to create a shorter version of it ~\cite{inbook}. In this research work, we propose a transformer-based method for selecting meaningful phrases from clinical discharge summaries and extracting them by preserving the sense of clinical notes based on the identified disease. Transformer~\cite{transformer} is being used as a new tool for text analysis tasks in NLP~\cite{bahdanau}. 
% It is a layered neural network-based architecture that exploits attention mechanism for supervised tasks. 
% Bidirectional Encoder Representation Transformer (BERT) contains 12 transformer layers and several multiple attention heads to form embeddings and attention tensors for a given sentence~\cite{DBLP:journals/corr/abs-1810-04805}. 
Inspired by~\cite{clinicalbert}, we have further tuned a BERT model utilizing discharge notes classified by diseases of the MIMIC-III dataset, Which captures important syntactic information based on International Classification of Diseases (ICD-9) labels. We extract a discrete attention distribution from the last layer. This probabilistic distribution is later translated using power transforms~\cite{book} to create monotonic data over bell curve~\cite{attentions}. 
% We choose the value from the first attention head of the last layer to create a series for identifying the importance of every sentence. 
Finally, the summary is comprised of sentences that have higher attention scores than the mean attention scores.\par

This paper organizes sections as follows: Section~\ref{sec:2} illustrates various types of extractive summarization approaches and their usescases on medical documents. In Section~\ref{sec:3}, we described the methodology for intended task.
% we introduce an attention-based method in the medical summarization domain trained on coding clinical notes.
Section~\ref{sec:4} presents various evaluation methods and states a suitable method for this task. We have displayed results in Section~\ref{sec:5}.
% with an insight into related work in Section \ref{sec:6}. 
Finally, we conclude the discussion in Section~\ref{sec:6} with limitations of interpretation in the medical domain in Section~\ref{sec:7}.\par


% ======================================================================
% =======================================================================
\section{Related Work} \label{sec:2}
The early works on summarization are based on many different surface-level approaches for the intermediate representation of text documents. These methods focus on selecting top sentences based on some greedy algorithms and aim for maximizing coherence and minimizing redundancy~\cite{Allahyari}~\cite{zhong2020extractive}. These techniques can be further generalized into:
\begin{itemize}
    \item \textbf{Corpus-based Approach:} It is a frequency-driven approach based on common words that are often repeated and do not carry salient information. It relies on an information retrieval paradigm in which common words are considered as query-words. SumBasic~\cite{Vanderwende} is a similar centroid-based method that uses word probability as a factor of importance for sentences. Words in each centroid with higher probabilistic values are selected for a summary. \par
    
    \item \textbf{Cohesion-based Approach:} Some techniques fail while extraction when the text is bound to anaphoric expressions. \footnote{ Anaphoric expressions are words that relate the sentences using pronouns such as he, himself, that.} Lexical chains are used to find a relation between two sentences. Brin et al.~\cite{Brin} proposed a co-reference system that uses cohesion for this purpose in web search. In clinical notes, anaphoric expressions are used frequently, but they refer to the same subjects meaning that we have a single relation to the patient. \par
    
    \item \textbf{Rhetoric-based Approach:} This method relies on forming text organization in a tree-like representation ~\cite{Goldstein}~\cite{Kupiec}. Text units are extracted based on their position close to the nucleus. For clinical summaries, we often may have multiple nuclei for different diseases.\par
    
    \item \textbf{Graph theoretic Approach:} A few popular algorithms like HITS~\cite{Knight} and Google`s PageRank~\cite{mihalcea} instigated base for graph-based summarization. It helps to visualize intra-topic similarity where nodes present a number of topics and vertices show their cosine similarity with sentences~\cite{gupta}. It makes visual representation easy with different tools like MDIGESTS~\cite{Chongtay}.\par
    
    \item \textbf{Machine Learning Approach:} ML models are outperforming for nearly all kinds of tasks, including text summarization. A recent trend of analyzing text using Bayesian models has gained popularity~\cite{Ayodele}. Neural networks better exploit hidden features from the text. Attention mechanism coupled with convolution layers helps to select importing phrases based on their position in the document. ML models treat summarization as a classification task. Transformer-based models combined with clustering methods are used in an unsupervised fashion. Miller et al.~\cite{miller2019leveraging} used BERT to make text encoding and applied K-means to find sentences close to the centroid to learn health-informatics lecture summaries. This model offered a weakness for large documents since the extraction ratio is fixed for K sentences. Liu et al.~\cite{liu2019fine} trained an extractive BERT model from abstractive summaries using a greedy method to generate an oracle summary for maximizing the ROGUE score. BERTSUM~\cite{liu2019fine} used a trigram blocking method to extract candidate sentences based on golden abstractive summaries in CNN/daily mail dataset. 
\end{itemize}


\subsection{Implementations for Medical Documents}
%\paragraph{Empirical Methods: } 
Clinicians heavily rely on text information to analyze the condition of the patient. Vleck et al.~\cite{Vleck} followed a  cognitive walk-through methodology by identifying certain relevant phrases to medical understanding. They developed a new extrinsic evaluation for the results. Laxmisan et al.~\cite{Laxmisan} formed a clinical summary screen to integrate with existing personal health record systems. The core purpose was to avail more interaction time for a clinician. \par


Feblowitz et al.~\cite{Feblowitz} proposed a five-stage architecture to facilitate clinical summarization tasks. It was more based on producing short laboratory reports. The AORTIS model was evaluated using cohesion index Kappa. The abbreviation of AORTIS described distinct phases of the framework, namely Aggregation, Organization, Reduction, Interpretation and Synthesis (AORTIS)~\cite{wright}. Alsentzer et al.~\cite{Alsentzer} did a similar job using Bayesian modeling. They utilized heterogeneous sampling and topic modeling stated in the research paper~\cite{Pivovarov}. They materialized a Concept Unique Identifier CUI-Upper bound to choose a phrase that has a high probability of being classified as a disease.\par

%\paragraph{Graphical Methods: } 
Thomas et al.~\cite{Thomas} presented a semi-supervised graph-based method for summarization using neural networks and node classification. The model was limited to datasets other than the clinical domain. Other researchers followed a similar kind of method, G-FLOW for Multi-document Summarization~\cite{Christensen}~\cite{Michihiro}. Azadani et al.~\cite{Azadani} carried out these ideas to biomedical summarization. They formulated a model based on graph clustering that forms a minimum spanning tree using Unified Medical Language System (UMLS).\par

An ontology-oriented graphical representation was proposed in this article~\cite{Yoo}. It described a clustering method that uses data centrality and mutual refinement to sample to limit compression. Mis-Classification index (MI), a new evaluation metric to verify cluster purity was used as primary evaluation. These implementations were done on different datasets and the organization of clinical notes. Generally, graphical methods concluded better results in most of the cases. 
% This paper proposes a
% % n innovative method for finding clinical summaries, unlike a traditional ML approach. We are using BERT architecture trained on the MIMIC dataset for ICD-9 coding to find 
% extractive summarization from clinical notes based on its word distribution and multi-head attention mechanism on label importance. The details can be read in Section~\ref{sec:3.2}.\par

\begin{figure*}[ht]
    \centering
    \includegraphics[width =0.95 \textwidth,height = 12cm ]{bert.pdf}
    \caption{BERT base architecture with 12 transformer layers. Every layer carries embeddings (blue) and attention scores (green) for corresponding tokens. This multi-head attention correlates to every other word as seen in the images at left. The classifier token from the last layer is used for every sentence are described in the methodology.}
    \label{fig:1}
\end{figure*}

%======================================================================
% =======================================================================


\section{Methodology} \label{sec:3}
We propose a method to extract important phrases from a clinical note. This approach uses a base BERT-model fined-tuned on ICD-9 labeled MIMIC-III discharge notes. The model was trained mainly to identify ICD-9 labels based on described symptoms and diagnosis information. This summarization approach works effectively when reference or human-made summaries are not available.
The model outputs attention scores for all sentences from discharge notes. We are extracting sentences whose attention scores are higher than the mean value of all other sentences in the original note. Our model is compared against three baselines ~\cite{Edmundson}~\cite{Michihiro}~\cite{miller2019leveraging} using divergence methods of word probability distributions for quantitative analysis. Table~\ref{results2} represents qualitative analysis against chosen baseline approaches. \par

\subsection{Dataset} \label{sec:3.1}
MIMIC-III is an open-access publicly available database of unstructured health records~\cite{Johnson}. This dataset is available online.\footnote{https://physionet.org/content/mimiciii-demo/1.4/} It includes raw notes of 36,998 patients for each hospital stay. Each discharge note is tagged with a unique label for the identified disease. In total, we have 47,724 clinical discharge notes that comprise several details from radiology, nursing, and prescription. These notes can be equated with a multi-topic document based on the nature of multiple labels for each medical note. 
% The BERT model is fine-tuned for discharge notes according to ICD-9 codes that score attention values over the tokens constituting the sentences.
A reduced sample of randomly selected 100 notes of this dataset is selected to quantitatively and qualitatively assess the performance of the model. 
% The sample has been selected randomly. 
The dataset was only published for labeling diagnostics and does not contain any kind of reference summary. \par


\subsection{Neural Architecture} \label{sec:3.2}
We have utilized neural architecture that is built on top of transformer~\cite{transformer}. Bidirectional Encoder Representation from Transformer (BERT) is multi-layer neural architecture. It has two major variants. We have used a base variant with 12 layers (transformer blocks), 768 hidden sizes, 12 attention heads, and 110 million parameters. The language model has shown significant improvements in various language processing tasks with fine-tuning~\cite{Howard}~\cite{Dai}. 
% We have adopted pre-trained weights and performed fine-tuning for the task of coding discharge notes. 
The BERT model usually creates embeddings in both directions for the representation of the inputs~\cite{DBLP:journals/corr/abs-1810-04805}. We have found that attention heads corresponding to delimiter tokens are remarkably effective for semantic understanding. This approach is trained using the classes available in the MIMIC-III dataset that map clinical notes to pathologies. \par

\subsection{Implementation Details}\label{sec:3.3}
The work presented in this paper employs fine-grained understanding of the notes to signify sentences that are relevant for the classification and brings more information to a summary. Finally, we have demonstrated attention scores for sentences using a highlighting tool (see Sec.~\ref{sec:3.4}) to inspect the output results. Figure \ref{fig:1} shows the model along with attention flow.\par


\paragraph{\textbf{Token Representation: }} A sentence flows downstream as a sequence of tokens accompanied by two special tokens. An input representation for any token is formed by combining token, position, and segment embedding. [CLS] is the first token that classifies a sentence and appears in the beginning. [SEP] is a separator token used to identify the end of the stream. At the output [CLS], representation can be fed to the classifier for various tasks. We have only used the corresponding attention head for the task of summarization.\par

\paragraph{\textbf{Pre-processing: }} Clinical documents contain many irregular abbreviations and periods for their particular formatting. Some fragments of notes are in grammatical order, whereas other parts are written as review keywords. We have used the custom tokenizer presented in~\cite{Mullenbach} to formulate data in a listed manner. It removes tokens that contain no alphabetic character and are used as a percentage of drug prescriptions. 
\par
% We have trimmed discharge notes which are longer than 3000 tokens.\par 

\paragraph{\textbf{Fine-Tunning: }} Fine-tuning has a huge effect on performance for supervised tasks~\cite{kovaleva}. We have fine-tuned BERT model %with a python index package simple-transformer\footnote{https://pypi.org/project/simpletransformers/} 
using maximum sequence length, batch size 8, learning rate 3e-5, ADAM optimizer with epsilon 1e-8, and keeping other hyper-parameters the same as that of pre-training. The fine-tuned model can be used to classify [CLS] token for maximum-likelihood of ICD-9 label. \par

\paragraph{\textbf{Attention Extraction: }}  Fine-tuning helps to encode semantic knowledge in self-attention patterns ~\cite{kovaleva}. 
% Training model on the same dataset creates a notional understanding of clinical notes.
Multi-head attention mechanism embeds every sentence of clinical note with a special token and feeds it to the first layer. Since the last layer of BERT model is considered vital to task-specific~\cite{van2019does}, we capture the first attention head of the last layer that is important for cross-sentence relation as observed with BertViz. This attention head focuses on a special [CLS] token. Attention scores from the first head of the last layer correspond to the whole sentence and are used as a measure of significance in a sentence.  
% Later, we decide to extract all those sentences whose weight is above the mean of all other intra-attention weights. 
Equation ~\ref{eq:1} and Equation ~\ref{eq:2} show how the dot-product attention is calculated in layers.\par

 \begin{equation}\label{eq:1}
      a_i = Softmax(f(Q,K_i)) = \frac{exp(f(Q,K_i))}{\sum _i exp(f(Q,K_i))}
 \end{equation}
 
 \begin{equation}\label{eq:2}
      Attention(Q,K,V) = \sum _i a_i\ast V_i
 \end{equation}
 
 A set of pre-processed clinical notes in the form of a list of sentences are fed to the BERT encoder, which creates embedding and attention scores at each layer. The attention score corresponding to [CLS] decides whether a sentence is a good candidate for the summary. Figure ~\ref{fig:2} illustrates the positional relevance of the [CLS] token. We have later selected sentences whose attention scores of the constituting words are above the average attention value of the original note. This extraction incentives dynamic selection, unlike a fixed sentence summary ratio.  For example, a sentence with an attention score of 0.14 is chosen if it is greater than the average of attentions of all sentences in the document.\par 
 
 \begin{figure}[t!]
    \centering
    \includegraphics[width=6.5cm]{bertviz.png}
    \caption{Attention Visualization shows how every attention-head in BERT architecture finds word useful to other words in a sentence. We have a different color for every head identifying its position in the last layer. This demonstration is performed using BertViz tool~ \cite{Vig}.}
    \label{fig:2}
\end{figure}


\subsection{Sentence Attention Visualization}\label{sec:3.4}
The attention distribution for tokens on the last layer has an irregular pattern. In order to perform a heat-mapping, we have utilized a tool namely Neat-Vision.\footnote{\url{https://github.com/cbaziotis/neat-vision}}

This tool requires a fixed type of input format and outputs a text heat-map. It demands input data be organized in a particular structure for vibrant coloring. We have stratified the distribution obtained from the neural architecture to the Gaussian distribution using the \textit{Quantile Transformation}~\cite{book}. This turns a sentence with great attention more fragrant in visibility and vice versa. In other words, it makes sentences with higher attention scores rosier than the other ones. Figure~\ref{fig:3} shows the impact of transformation on attention series data. Here x-axis presents the number of sentences, and the y-axis accounts for the value of the attention score for the corresponding sentence. This demonstration will have a huge impact on clinician practice by alienating time spent while reading long health records. Figure ~\ref{fig:4} exhibits the usefulness of heat-mapping concepts for health systems.\par

\begin{figure}[t]
    \centering
    % \includegraphics[width=7cm]{quantile.pdf}
    \includegraphics[width=7cm]{png2pdf.pdf}
    \caption{Effect of quantile transform on attention scores of all sentence in the document. The red line shows obtained attention distribution with a low variance where as the blue line shows higher variance that can be efficiently utilized for heat-mapping.}
    \label{fig:3}
\end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=8cm]{heatmapping.png}
 \caption{An excerpt of heat-mapping on Neat-Vision tool with transformed attention values to highlight importance of sentence with red color.}
 \label{fig:4}
\end{figure}


%======================================================================
%=======================================================================


\section{Evaluation} \label{sec:4}
Evaluation in summarization has been a critical issue, mainly due to the absence of a gold standard. Many competitions such as DUC \footnote{\url{http://duc.nist.gov/}} ,TREC\footnote{ \url{http://trec.nist.gov/}}, SUMMAC\footnote{\url{https://www-nlpir.nist.gov/related_projects/tipster_summac/}} and MUC\footnote{\url{http://www.itl.nist.gov/iad/894.02/related projects/muc/proceedings/muc 7 toc.html}} propose different metrics. The interpretation of these metrics is not so simple, mainly because the same summary receives different scores under different measures. Automatic evaluation for the quality of the summary is an ambitious task and can be performed by making a comparison with a human-generated summary. For this reason, evaluation is normally limited to domain-specific and opinion-oriented areas~\cite{inbook}.\par

Formally, these evaluation methods can be divided into two areas. In \textit{extrinsic} evaluation, it is manually analyzed how useful the summary is for the supplied document. For instance, this can be done by a clinician in our case and may result in different opinions based on his understanding. Miller et al.~\cite{miller2019leveraging} leveraged this manual clinical evaluation to compare the performance of their model. In \textit{intrinsic} evaluation, the extracted summary is directly matched with the ideal summary created by humans. The latter can be divided into two classes, primarily because it is hard to establish an ideal reference summary by a human. 
\begin{itemize}
\item \textit{Text quality Evaluation:} It is more related to linguistic check that examines grammatical and referential clarity. This assessment is not complete predominately owing to the fact that medical summaries are unstructured documents with lots of abbreviations and clinical jargon.
\item \textit{Content-based Evaluation:} It rates summaries based on provided reference summaries ~\cite{steinberger}. Some of the common approaches are ROGUE (Recall-Oriented Understudy for Gisting Evaluation) ~\cite{Lin}, Cosine Similarity and Pyramid Method ~\cite{nenkova2007pyramid}. Liu et al.~\cite{liu2019fine} studied unigram and bigram ROGUE overlaps for different components of BERTSUM for their single-document summaries.
\end{itemize}

Sripada et al.~\cite{sripada} in their work presented that a summary can be considered effective if it has a similar probability distribution as that of the original document. The hypothesis was compared in other research works~\cite{nenkova} ~\cite{yih} where this light-weight and less complex method demonstrated finer results. This criterion is a more suitable evaluation for our methodology since we do not have the reference summaries in MIMIC dataset. We will compare the distribution of words in the original and summary document to identify their effectiveness. We will use two tests for evaluating the goodness of our synopsis, namely Kullback–Leibler divergence (KLD) ~\cite{KLD} and Jensen–Shannon divergence (JSD)~\cite{JSD}.\par

\paragraph{KL Divergence:} It is a measure of the difference between two distributions. This measure is asymmetric, and the minimum KLD value shows better relative interference for distributions; for discrete probability distributions P and Q mapped on probability space $\zeta$, KLD from Q to P is defined in Equation ~\ref{eq:3} ~\cite{das}; \par

\begin{equation}\label{eq:3}
\centering
\Large{KLD(P || Q) = \sum_{x\epsilon\zeta}P(x)\log{\frac{P(x)}{Q(x)}}}  
\end{equation}

\paragraph{JS Divergence:} It is an extension of KL divergence that quantifies the difference in a slightly modified way. It is a smoothed and normalized form assuring symmetry among inputs as reported in Equation ~\ref{eq:4}~\cite{JSD}.\par

\begin{equation}\label{eq:4}
\centering
\large
{JSD(P || Q) = \frac{1}{2}KLD(P || M) + \frac{1}{2}KLD(Q || M).}  
\end{equation}
where, \par

\begin{equation}\label{eq:5}
\centering
 M = \frac{1}{2} (P + Q)
\end{equation}


%======================================================================
%=======================================================================


\section{Results} \label{sec:5}
We have performed a comparison of our model with three baselines for extractive summarization methods. First, Part-of-Speech-based sentence tagging is designed on the empirical frequency selection method. The second one centers around the graphical method, and the third one uses BERT combined with K-means to find top k sentences. The results can be reproduced, and source code for replication is available on our Github repository.

% ~\footnote{\url{https://github.com/NeelKanwal/BERTOLOGY-Based-Extractive-Summarization-for-Clinical-Notes}}.\par

The proposed architecture shows significant improvement compared with baseline approaches. Divergence scores significantly show how estimating differences in distributions can help in anticipating the word distribution of both documents. Table ~\ref{results1} exhibits that our extracted summaries are more informative than others based on lower average of KL and JS divergence scores. Frequency-based approach outcomes highest divergence among others. JSD and KLD scores for the graph-based method show a relative amelioration compared to frequency-based methods. There is a little quantitative difference of values with the centroid-based approach due to their nature of calculating sentence embeddings in a similar way. Our method is dynamic in choosing the length of the summary, which overcomes the weakness of fixed K sentences described in the paper~\cite{miller2019leveraging}. Overall, the attention mechanism poses great abstraction power for the summarization task.\par


\begin{figure}[t]
 \centering
 \includegraphics[width=8.5cm,height=6.5cm]{jsd_new.pdf}
 \caption{Line chart for JSD values for experimented models over sampled-set of clinical notes from MIMIC-III dataset.}
 \label{fig:5}
\end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=8.5cm,height=6.5cm]{kld_new.pdf}
 \caption{Line chart for KLD values for experimented models over sampled-set of clinical notes from MIMIC-III dataset.}
 \label{fig:6}
\end{figure}


\begin{table}[h!]
    \large\centering
 \begin{tabular}{|l| c c |}
    \hline
    Models & \textbf{KLD$\downarrow$} & \textbf{JSD$\downarrow$}\\
    \hline \hline
    Frequency-Based Approach & 0.892 & 0.426  \\
    Graph-Based Approach & 0.827 & 0.408  \\
    Centroid-Based K-means Approach & 0.80 & 0.41 \\
    \textbf{Our Proposed Architecture} & \textbf{0.795} & \textbf{0.405} \\[0.5ex]
    \hline
    \end{tabular}
    \caption{Experimental results on a reduced sample-set of 100 random clinical notes from MIMIC-III dataset compared with Frequency-Based Approach ~\cite{Edmundson}, Graph-Based Approach ~\cite{Michihiro} and Centroid based K-means Approach~\cite{miller2019leveraging} using KLD and JSD Values. A lower value pertains to a better-correlated summary.}
    \label{results1}
\end{table}



\begin{table*}[t]

\begin{tabular}{|| p {17cm} ||}
\hline\hline
\vspace{0.5em}\textbf{Centroid-Based K-means Summary: }daily disp tablet delayed release e.c. lastnametoken on february at 15pm cardiologist dr. lastnametoken on february at 30am wound check on thurs january at am with cardiac surgery on hospitaltoken please call to schedule appointments with your primary care dr. lastnametoken in march weeks please call cardiac surgery office with any questions or concerns telephonenumbertoken answering service will contact on call person during off hours completed by january.\newline\\

\textbf{Frequency-Based Summary: }disp tablet refills ranitidine hcl mg tablet sig one tablet daily. refills tramadol tablet two tablet q6h hours as needed for pain. tablet senna mg tablet  One tablet daily, disp tablet refills furosemide mg tablet for Mitral valve repair coronary artery bypass. graft x left internal mammary artery to left anterior descending history of present illness year old female who was told she had mvp since age currently quite active but has noticed some dyspnea on exertion when walking up hills most recent echo revealed severe mvp and moderate to severe Daily daily disp tablet delayed release e.c. s refills docusate sodium mg capsule sig one capsule po bid times Disp tablet er particles crystals s refills discharge disposition home with service facility hospitaltoken vna discharge diagnosis mitral regurgitation coronary artery  disease. \newline\\

\textbf{Graph-Based Summary: }refills docusate sodium mg capsule one capsule a day magnesium hydroxide suspension thirty ml at bedtime as needed for constipation atorvastatin tablet one tablet daily. disp tablet s refills furosemide tablet once a day for days disp tablet refills ranitidine hcl mg tablet daily.
please shower daily including washing incisions gently with mild soap no baths or swimming until cleared by surgeon look at your incisions daily for redness or drainage. please no lotions cream powder or ointments to incisions each morning you should weigh yourself and then in the evening take your temperature these should be written down on the chart no driving for approximately one month and while taking narcotics will be discussed at follow up appointment with surgeon when you will be able to drive no lifting more than pounds for weeks please call with any questions or concerns telephonenumbertoken females please wear bra to reduce pulling on incision avoid rubbing on lower edge. please call cardiac surgery office with any questions or concerns telephonenumbertoken answering service will contact on call person during off hours followup instructions you are scheduled for the following appointments surgeon dr. lastnametoken on february at 15pm cardiologist dr. lastnametoken on february at 30am wound check on thurs january at am with cardiac surgery on hospitaltoken.\newline \\

\textbf{Our Proposed Approach: }old female who was told she had mvp currently quite active but has noticed some dyspnea on exertion when walking up hills. she presents for surgical consultation past medical history mitral regurgitation copd secondary to asbestos exposure as a child arhtritis cataracts headaches lactose intolerance r wrist and elbow surgery. widowed occupation retired disabled nurse tobacco quit smoking in father died suddenly at cause unknown physical exam. no spontaneous echo contrast is seen in the left atrial appendage there is a small pfo with left to right flow overall left ventricular systolic function is normal lvef in the face of mr there is normal free wall contractility there are simple atheroma in the descending thoracic aorta the aortic valve leaflets are mildly thickened trace aortic regurgitation is seen the posterior leaflet is very degenerate and there is moderate to severe mitral regurgitation. there is no pericardial effusion the tip of the sgc is seen at the pa bifurcation post cpb the patient is av paced on no inotropes the pfo is closed normal biventricular systolic fxn there is a mitral ring prosthesis which is well seated trace mr residual mean gradient with an area of no ai aorta intact. mrs. lastnametoken was a same day admit after undergoing all pre operative work. she was tolerating a full oral diet her incisions were healing well and she was ambulating in the halls without difficulty it was felt that she was safe for discharge home at this time with vna services all appopriate follow up appointments were arranged.\newline \\

\hline \hline
\end{tabular}
\caption{Qualitative Analysis For Different Approaches}
\label{results2}
\end{table*}

As noted in Figure~\ref{fig:5} and ~\ref{fig:6}, there are some summaries where distributional similarity does not outperform in cases where clinical notes are shorter in length. The curve presents that attention-based extraction is more impactful than other counterparts. JS divergence metrics show less fluctuation than other the metric because of its averaging symmetry mechanism. 
Summaries from each method are placed in Table~\ref{results2} for qualitative analysis. It can be observed that summaries generated by our proposed architecture have more coherence and make it easier to adapt clinical understanding. On the other hand, baselines approaches provide short and incoherent sentences for the selected note. Shorter summaries are more likely to lose discriminatory information and affect the degree of understanding; thus, evaluating the usefulness of a summary in terms of sentences may not be optimal.  As described in Section ~\ref{sec:4}, it may be hard for a non-specialist to understand the relative usefulness of each summary. This method shows the applicative benefits of dynamic summarization in healthcare systems.  Furthermore, it is more helpful for a physician to grab the essence of diagnosis via highlighting tools as displayed in figure~\ref{fig:4}. \par
%======================================================================
%=======================================================================



\section{Conclusion} \label{sec:6}
The immense increase in digital text information has certainly emphasized the need for universal summarization frameworks. Abstractive summarization has been an area of research debatable for certain scenarios, e.g., medical, because of the risk of generating summaries that deliver different meanings of the original notes reported by physicians. 
% Despite various frameworks, completely resolving intrinsic ambiguity in the medical text can be hard with traditional approaches.
Extractive summarization techniques are relatively reasonable in the clinical domain. Research interest in creating synopsis has been re-surged after the advent of machine learning techniques. 
Evaluation in medical summarization is at the toughest degree compared to other domains. 
% A physician who authored a discharge note may find the obtained summary helpful. On the other hand, a physician who is not familiar with patient history may find it dull in explanation.
We have utilized statistical analysis methods to understand the magnitude of relevance between summary and original clinical notes. The evaluation criteria of finding divergence among distributions are suitable when ideal summaries are not present. \par
In this paper, we have elucidated a neural architecture for extracting summaries based on multi-head attentions. The proposed model is domain-specific and outperforms other methods debated in the literature. The architecture achieves better results on a set of MIMIC-III clinical notes, outperforming frequency, graph-oriented, and centroid-based approaches. Furthermore, our proposed model can be integrated into a decision-support system to provide a better interpretation of clinical information by highlighting diagnostically related phrases.\par


%======================================================================
%=======================================================================


\section{Limitations and Future Work} \label{sec:7}
Medical summarization is a special and delicate task. It is quite hard to evaluate whether the obtained summary is a general well-condensed representation of the document, and it would require manual labor and a trial with physicians for a clinical assessment. Moreover, performing a qualitative evaluation is subjective and may highly depend on the physician's personal experience of dealing with similar diseases. 

The utilized clinical attention-based model is fine-tuned on the MIMIC-III dataset. Therefore, it may not perform well on a different kinds of clinical notes, written in a different structure and mapped onto a different set of diseases. ICD-9 offers wide coverage and accurate cataloging; however, we are considering ICD-10 in current research activities.
As future work, a concoction of abstractive and extractive summarization using a neural network language generation model may be more bankable. A universal medical summarizer may omit limitations arising from diverse writing style and reduce computational complexity.
